Research Borderlands: Analysing Writing Across Research Cultures

Improving cultural competence of language technologies is important. However most recent works rarely engage with the communities they study, and instead rely on synthetic setups and imperfect proxies of culture. In this work, we take a human-centered approach to discover and measure language-based cultural norms, and cultural competence of LLMs. We focus on a single kind of culture, research cultures, and a single task, adapting writing across research cultures. Through a set of interviews with interdisciplinary researchers, who are experts at moving between cultures, we create a framework of structural, stylistic, rhetorical, and citational norms that vary across research cultures. We operationalise these features with a suite of computational metrics and use them for (a) surfacing latent cultural norms in human-written research papers at scale; and (b) highlighting the lack of cultural competence of LLMs, and their tendency to homogenise writing. Overall, our work illustrates the efficacy of a human-centered approach to measuring cultural norms in human-written and LLM-generated texts.

==> v1/tables/feature_operationalizations.tex <==
\begin{table*}[t]
    \centering
    \footnotesize
    \begin{tabular}{ll}
        \toprule
        \multicolumn{2}{c}{Structural Norms}\\
        \midrule
        \textbf{Length} & word and sentence count tokenized with NLTK and cleaned for special characters \\
        \textbf{Tables and Figures} & regex matches to customized lexicon (A\ref{appendix:artifacts}) \\
        \midrule
        \multicolumn{2}{c}{Vocabulary and Style} \\
        \midrule
        \textbf{Jargon} & lexical specificity scores \citep{zhang2017community,lucy-etal-2023-words} \\
        \textbf{Formality} & formality classifier from \cite{dementieva-etal-2023-detecting} \\
        \textbf{Readbililty} & Flesch reading-ease scores using \href{https://github.com/textstat/textstat}{https://github.com/textstat/textstat} \\
        \midrule
        \multicolumn{2}{c}{Rhetorical Elements} \\
        \midrule
        \textbf{Quantitative Evidence} &  LLM-as-judge setup with Llama 3.1 70B Instruct (A\ref{appendix:quant})  \\
        \textbf{Narrative Organization} & positional skew of background, objectives, methods, and findings using \citet{fok2023scim} \\
        % \textbf{Metaphorical Motifs} &   \\
        \textbf{Framing} & lexicon to capture ten \textit{values} encoded in sentences from \citet{birhane2022values} \\
        \bottomrule
    \end{tabular}
    \caption{
        Operationalizations of features discovered in our qualitative study. See the Appendix for additional background and implementation details.}
    \label{table:feature-operationalizations}
\end{table*}

